Cyclic Mutually Unbiased Bases and Quantum Public-Key Encryption

The thesis is mainly about the construction and implementation of cyclic mutually unbiased bases, dealing with different entanglement structures by discussing the related group structures. A recursive construction for Fermat number dimensions is given and related to Wiedemann's conjecture for systems with more than 2048 qubits. The second part of the thesis analyses a quantum public-key encryption scheme.

==> odd_dimensions.tex <==
Results of Gow \cite{Gow07} indicate, that complete sets of MUBs cannot be generated
cyclically for odd prime-power dimensions $d=p^m$ with an odd prime $p \in \N$ and $m \in N$.
Nevertheless, we fo
